Technical Report: Multi-Carrier Position-Based Packet Forwarding Protocol For Wireless Sensor Networks

Beaconless position-based forwarding protocols have recently evolved as a promising solution for packet forwarding in wireless sensor networks. However, as the node density grows, the overhead incurred in the process of relay selection grows significantly. As such, end-to-end performance in terms of energy and latency is adversely impacted. With the motivation of developing a packet forwarding mechanism that is tolerant to node density, an alternative position-based protocol is proposed in this paper. In contrast to existing beaconless protocols, the proposed protocol is designed such that it eliminates the need for potential relays to undergo a relay selection process. Rather, any eligible relay may decide to forward the packet ahead, thus significantly reducing the underlying overhead. The operation of the proposed protocol is empowered by exploiting favorable features of orthogonal frequency division multiplexing (OFDM) at the physical layer. The end-to-end performance of the proposed protocol is evaluated against existing beaconless position-based protocols analytically and as well by means of simulations. The proposed protocol is demonstrated in this paper to be more efficient. In particular, it is shown that for the same amount of energy the proposed protocol transports one bit from source to destination much quicker.

==> bibfileshorte.bib.tex <==
@ARTICLE{mesh.survey.Akyilidiz,
  AUTHOR =       "I. Akyildiz and X. Wang and W. Wang",
  TITLE =        "Wireless mesh networks: a survey",
  JOURNAL =      "Elsevier Journal on Computer Networks",
  YEAR =         "2004",
  volume =       "47",
  number =       "4", 
}

@ARTICLE{wsn.survey.Akyilidiz,
  AUTHOR =       "I. Akyildiz and W. Su and Y. Sankarasubramaniam and E. Cayirci",
  TITLE =        "Wireless sensor networks: a survey",
  JOURNAL =      "Elsevier Journal on Computer Networks",
  YEAR =         "2002",
  volume =       "38, Issue 4",
}

@ARTICLE{linear.clock.drift,
  AUTHOR =       "M. Sichitiu and C. Veerarittiphan",
  TITLE =        "Simple, Accurate Time Synchronization for Wireless Sensor Networks",
  JOURNAL =      "IEEE Wireless Communications and Networking Conference, WCNC",
  YEAR =         "2003",
  volume =       "2",
  pages =        "1266-1273",
  month =        "March",
}

@BOOK{mob.comm.Hagenauer,
  AUTHOR =       "J. Hagenauer",
  TITLE =        "Mobile Communications",
  PUBLISHER =    "lecture notes, Insitute for Communications Engineering, Munich University of Technology",
  YEAR =         "2005",
}

@ARTICLE{MIMOOFDM.multihopMAC.Wang,
  AUTHOR =       "Dandan Wang and Uf Tureli",
  TITLE =        "Joint MIMO-OFDM and MAC Design for Broadband Multihop Ad Hoc Networks",
  JOURNAL =      "EURASIP Journal on Wireless Communications and Networking",
  YEAR =         "2006",
  volume =       "2006",
  number =       "60585",
  month =        "June",
}

@ARTICLE{MIMAMAC.multihop.Tang,
  AUTHOR =       {T. Tang and M. Park and R. Heath, Jr. and S. Nettles},
  TITLE =        "Joint MIMO-OFDM Transceiver and MAC Design for Mobile Ad Hoc Networking",
  JOURNAL =      "Proc. of Int'l Workshop on Wireless Ad-Hoc Networks, Oulu, Finland",
  YEAR =         "2004",
  month =        "June",
}

@ARTICLE{dualBTMA.adhoc.Haas,
  AUTHOR =       "Z. J. Haas and J. Deng",
  TITLE =        "Dual busy tone multiple access (DBTMA) - a multiple access control scheme for ad hoc networks",
  JOURNAL =      "IEEE Transactions on Communications",
  YEAR =         "2002",
  volume =       "50",
  number =       "6",
  pages =        "975-985",
}

@ARTICLE{BMAC.Berkeley,
  AUTHOR =       "J. Polastre and J. Hill and D. Culler",
  TITLE =        "Versatile low power media access for wireless sensor networks",
  JOURNAL =      "SenSys 04: Proceedings of the 2nd international conference on embedded networked sensor systems",
  YEAR =         "2004",
  pages =        "95-107",
}

@ARTICLE{SMAC.Goldsmith,
  AUTHOR =       "W. Ye and J. Heidmann and D. Estrin",
  TITLE =        "An energy-efficient mac protocol for wireless sensor networks",
  JOURNAL =      "Proceedings of the 21st Interntional Annual Joint Conference of the IEEE Computer and Communictions Societies (INFOCOM 2002)",
  YEAR =         "2002",
  month =        "June",
}

@ARTICLE{TMAC.VanDam,
  AUTHOR =       "T. van Dam and K. Langendoen",
  TITLE =        "An adaptive energy-efficient mac protocol for wireless sensor networks",
  JOURNAL =      "Proceedings of the first internation conference on embedded networked sensor systems",
  YEAR =         "2003",
  pages =        "171-180",
}

@ARTICLE{OFDM.extensions.Siemens,
  AUTHOR =       "M. Lott and A. Weckerle and W. Zirwas and H. Li and E. Schulz",
  TITLE =        "Hierarchical cellular multihop networks",
  JOURNAL =      "Proc. of 5th European Personal Mobile Communications Conference, Glasgow, UK",
  YEAR =         "2003",
  pages =        "37-43",
  month =        "April",
}

@BOOK{applications.OFDM,
  AUTHOR =       "H. Schulze and C. Lueders",
  TITLE =        "Theory and Applications of OFDM and CDMA",
  PUBLISHER =    "John Wiley and Sons Ltd",
  YEAR =         "2005",
  edition =      "1st",
}

@BOOK{wireless.communications.Goldsmith,
  AUTHOR =       "Andrea Goldsmith",
  TITLE =        "Wireless Communications",
  PUBLISHER =    "Cambridge University Press",
  YEAR =         "2005",
  edition =      "1st",
}

@ARTICLE{multicarrier.singlecarrier.Wang,
  AUTHOR =       "Z. Wang and X. Ma and G. Giannakis",
  TITLE =        "OFDM or Single-Carrier Block Transmission?",
  JOURNAL =      "IEEE Transactions on Communications",
  YEAR =         "2004",
  volume =       "52",
  number =       "3",
  pages =        "380-394",
  month =        "March",
}

@ARTICLE{sum.RayleighRV.Beaulieu,
  AUTHOR =       "N. C. Beaulieu",
  TITLE =        "An infinite series for the computation of the complementary probability distribution function of a sum of independent random variables and its application to the sum of Rayleigh random variables",
  JOURNAL =      "IEEE Transactions on Communications",
  YEAR =         "1990",
  volume =       "38",
  number =       "10",
  pages =        "1463-1474",
  month =        "September",
}

@ARTICLE{adaptive.loading.Chow,
  AUTHOR =       "P.S. Chow and J.M. Cioffi and John A.C. Bingham",
  TITLE =        "A practical discrete multitone transceiver loading algorithm for data transmission over spectrally shaped channels",
  JOURNAL =      "IEEE Transactions on Communications",
  YEAR =         "1995",
  volume =       "48",
  pages =        "772-775",
}

@Article{routing.fading.Haenggi,
  author =   {M. Haenggi},
  title =    {On Routing in Random Rayleigh Fading Networks},
  journal =   {IEEE Transactions on Wireless Communications},
  year =     {2005},
 volume = {4, no. 4}
}

@ARTICLE{subcarrier.assignment.Hottinnen.pdf,
  AUTHOR =       "Ari Hottinen and Tiina Heikkinen",
  TITLE =        "Subchannel assignment in OFDM relay nodes",
  JOURNAL =      "Proceedings of Conference on Information Sciences and Systems",
  YEAR =         "2006",
  month =        "March",
}

@BOOK{fadingbook,
  AUTHOR =       "M. Simon and M.S. Alouini",
  TITLE =        "Digital Communication over Fading Channels",
  PUBLISHER =    "John Wiley and Sons",
  YEAR =         "2005",
  edition =      "2nd",
}

@Article{empty.distance.Ekici,
  author =   {S. Vural and E. Ekici},
  title =    {Analysis of Hop-distance Relationship in Spatially Random Sensor Networks},
  journal =      {Proceedings of ACM Mobihoc 2005},
  year =     {2005},
}

@ARTICLE{performance.multihop.Hasna,
  AUTHOR =       "Mazen O. Hasna and Mohamed-Slim Alouini",
  TITLE =        "Performance Analysis and Optimization of Multihop Communication Systems",
  JOURNAL =      "Wireless communications systems and networks",
  YEAR =         "2004",
  pages =        "443-472",
}

@BOOK{digitalcomm.Proakis,
  AUTHOR =       "John G. Proakis",
  TITLE =        "Digital Communications",
  PUBLISHER =    "McGraw Hill",
  YEAR =         "2001",
  edition =      "4th",
}

@BOOK{convex.optimization,
  AUTHOR =       "S. Boyd and L. Vandenberghe",
  TITLE =        "Convex Optimization",
  PUBLISHER =    "Cambridge University Press",
  YEAR =         "2004",
}

@ARTICLE{probabilistic.mac.Haenggi,
  AUTHOR =       "M. Haenggi",
  TITLE =        "Probabilistic Analysis of a Simple MAC Scheme for Ad Hoc Wireless Networks",
  JOURNAL =      "IEEE CAS Workshop on Wireless Communications and Networking",
  YEAR =         "2002",
}

@ARTICLE{outage.cellularpackets.Rutgers,
  AUTHOR =       "Narayan B. Mandayam, Pi-Chun Chen and Jack M. Holtzman",
  TITLE =        {{Minimum Duration Outage for Cellular Systems: A Level Crossing Analysis}},
  JOURNAL =      "Proc. IEEE Vehicular Technology Conference",
  YEAR =         "1996",
  volume =       "2",
  pages =        "879-883",
}

@ARTICLE{minduration.outage.Rutgers,
  AUTHOR =       "Jie Lai and Narayan B. Mandayam",
  TITLE =        {{Minimum Duration Outages in Rayleigh Fading Channels}},
  JOURNAL =      "Proc. 31st Annual Conference on Information Sciences and Systems (CISS'97)",
  YEAR =         "1997",
}

@BOOK{wireless.book.Rappaport,
  AUTHOR =       "T. Rappaport",
  TITLE =        "Wireless Communications: Priciples and Practice",
  PUBLISHER =    "Prentice Hall",
  YEAR =         "2001",
  edition =      "2nd",
}

@ARTICLE{diversity.adhoc.Haenggi,
  AUTHOR =       "Martin Haenggi",
  TITLE =        "Analysis and Design of Diversity Schemes for Ad Hoc Wireless Networks",
  JOURNAL =      "IEEE Journal On Selected Areas In Communications",
  YEAR =         "2005",
  volume =       "23, Issue 1",
  number =       "",
  month =        "January",
}

@ARTICLE{fading.spectrum.Clarke,
  AUTHOR =       "R. Clarke",
  TITLE =        "A Statistical Theory of Mobile-Radio Reception",
  JOURNAL =      "BSTJ",
  YEAR =         "1977",
  volume =       "47",
  pages =        "957 - 1000",
 }

@BOOK{adaptive.filter.Haykin,
  AUTHOR =       "Simon Haykin",
  TITLE =        "Adaptive Filter Theory",
  PUBLISHER =    "Prentice Hall",
  YEAR =         "1996",
  edition =      "3rd",
}

@ARTICLE{blockfading.channel.Knopp,
  AUTHOR =       "R. Knopp, P.A. Humblet",
  TITLE =        "Maximizing Diversity on Block-Fading Channels",
  JOURNAL =      "IEEE International Conference on Communications",
  YEAR =         "1997",
  volume =       "2",
  pages =        "647-651",
  month =        "June",
}

@ARTICLE{multirelay.strategy.Sayed,
  AUTHOR =       "N. Khajehnouri and A. H. Sayed",
  TITLE =        "Multi-relay strategy for imperfect channel information in sensor networks",
  JOURNAL =      "to appear in Proc. EUSIPCO Antalya, Turkey",
  YEAR =         "2005",
  month =        "Sep",
}

@ARTICLE{semidefinite.relaxations.Parrilo,
  AUTHOR =       "P.A. Parrilo",
  TITLE =        "Semidefinite Programming Relaxations For Semialgebaic Problems",
  JOURNAL =      "Mathematical Programming Series B",
  YEAR =         "2003",
  volume =       "96",
  number =       "2",
  pages =        "293-320",
}

@ARTICLE{num.nonconcave.Fazel,
  AUTHOR =       "M. Fazel and M. Chiang",
  TITLE =        "Network Utility Maximization with Nonconcave Utilities Using Sum-of-Squares Method ",
  JOURNAL =      "To appear in Conference on Decision and Control",
  YEAR =         "2005",
  month =        "Dec",
}

@ARTICLE{genetic.search.Hajela,
  AUTHOR =       "P. Hajela",
  TITLE =        "Genetic Search - An Approach to the Nonconvex Optimization Problem",
  JOURNAL =      "AIAA Journal",
  YEAR =         "1990",
  volume =       "28",
  number =       "7",
  pages =        "1205-1210",
  month =        "July",
}

@ARTICLE{stochastic.nonconvex.Styblinski,
  AUTHOR =       "M. Styblinski and T. Tang",
  TITLE =        "Experiments in nonconvex optimization: stochastic approximation with function smoothing and simulated annealing",
  JOURNAL =      "ACM Journal on Neural Networks",
  YEAR =         "1990",
  volume =       "3, Issue 4",
  pages =        "467-483",
}

@Article{multihop.capacity.Kumar,
  author =   {P. Gupta and P. R. Kumar},
  title =    {The Capacity of Wireless Networks},
  journal =      {IEEE Transactions on Information Theory},
  year =     {2000},
  volume =   {46, Issue 2},
  pages =    {388-404},
  month =    {March},
}

@Article{capacity.bounds.Kumar,
  author =   {A. Agarwal and P.R. Kumar},
  title =    {Capacity Bounds for Ad hoc and Hybrid Wireless Networks},
  journal =      {ACM SIGCOMM Computer Communications Review},
  year =     {2004},
  volume =   {34},
  number =   {3},
  pages =    {71-81},
  month =    {July},
}

@ARTICLE{improved.bounds.Kumar,
  AUTHOR =       "A. Agarwal and P. R. Kumar",
  TITLE =        "Improved Capacity Bounds for Wireless Networks",
  JOURNAL =      "Wireless Communications and Mobile Computing",
  YEAR =         "2004",
  volume =       "4",
  number =       "Issue 3",
  pages =        "251-261",
  month =        "May",
}

@ARTICLE{fading.infotheory.Proakis,
  AUTHOR =       "E. Biglieri, J. Proakis, and S. Shamai (Shitz)",
  TITLE =        "Fading Channels: Information-Theoretic and Communications Aspects",
  JOURNAL =      "IEEE Transactions on Information Theory",
  YEAR =         "1998",
  volume =       "44, issue 6",
  pages =        "2619-2692",
}

@ARTICLE{transportcapcity.fading.Kumar,
  AUTHOR =       "F. Xue, L. Xie, and P. R. Kumar",
  TITLE =        "The Transport Capacity of Wireless Networks over Fading Channels",
  JOURNAL =      "IEEE Transactions on Information Theory",
  YEAR =         "2005",
  volume =       "51, Issue 3",
  month =        "March",
}

@ARTICLE{wsn.survey.GTech,
  AUTHOR =       "I.F. Akyilidiz, W. Su, Y. Sankarasubramaniamm and E. Cayirci",
  TITLE =        "Wireless Sensor Networks: A Survey",
  JOURNAL =      "Elsevier Journal on Computer Networks",
  YEAR =         "2002",
  volume =       "Vol 38",
  pages =        "393-422",
}

@Article{capacity.3classes.Toumpis,
  author =   {S. Toumpis},
  title =    {Capacity Bounds for Three Classes of Wireless Networks: Asymmetric, Cluster, and Hybrid},
  journal =   {Proceedings of the 5th ACM international symposium on Mobile ad hoc networking and computing},
  year =     {2004},
  pages =     {133-144},
}

@Article{capacity.regions.Toumpis,
  author =   {S. Toumpis and A. J. Goldsmith},
  title =    {{Capacity Regions for Wireless Ad Hoc Networks}},
  journal =      {{IEEE Transactions on Wireless Communications}},
  year =     {2003},
  volume =    {2, Issue 4},
  pages =     {736-748},
  month =     {July},
}

@Article{scaling.laws.Elgamal,
  author =   {H. El Gamal},
  title =    {{On The Scaling Laws of Dense Wireless Sensor Networks: The Data Gathering Channel}},
  journal =  {IEEE Transactions on Information Theory},
  year =     {2005},
  volume =   {51},
  pages =    {1229-1234},
  month =    {March},
}

@Article{cooperative.wsn.Rutgers,
  author =   {L. Sankaranarayanan and G. Kramer and N.B. Mandayam},
  title =    {{Hierarchical Sensor Networks: Capacity Bounds and Cooperative Strategies using the Multiple-Access Relay Channel Model}},
  journal =  {Proceedings of IEEE Conf. on Sensor and Ad Hoc Communication and Networks (SECON 2004)},
  year =     {2004},
  month =    {October},
}

@Article{capacity.routing.EPFL,
  author =   {G. Barrenechea and B. Beferull-Lozano and M. Vetterli},
  title =    {{Lattice Sensor Networks: Capacity Limits, Optimal Routing and Robustness to Failures}},
  journal =   {Proc. of 3rd International Symposium on Information Processing in Sensor Networks, IPSN 2004},
  year =     {2004},
  month =    {April},
}

@ARTICLE{dsss.interference.Sousa,
  AUTHOR =       "E. S. Sousa and J. A. Silvester",
  TITLE =        {{Optimum Transmission Ranges in a Direct-Sequence Spread-Spectrum Multihop Packet Radio Network}},
  JOURNAL =      "IEEE Journal on Selected Areas in Communications",
  YEAR =         "1990",
  volume =       "8, Issue 5",
  pages =        "762-771",
  month =        "June",
}

@ARTICLE{erristor.theory.Haenggi,
  AUTHOR =       "M. Haenggi",
  TITLE =        "Toward a circuit theory for sensor networks with fading channels",
  JOURNAL =      "Proceedings of the 2004 International Symposium on Circuits and Systems ISCAS '04",
  YEAR =         "2004",
  volume =       "4",
  number =       "IV",
  pages =        "908-911",
  month =        "May,
}

@Article{interference.multihop.Hekmat,
  author =   {R. Hekmat and P. Mieghem},
  title =    {{Interference in Wireless Multi-Hop Ad-Hoc Networks and Its Effect on Network Capacity}},
  journal =      {Wireless Networks},
  year =     {2004},
  volume =    {10},
  number =    {4},
  pages =    {389-399},
  month =     {July},
}

@Article{interference.graph.Microsoft,
  author =   {K. Jain and J. Padhye and V. Padmanabhan and L. Qiu},
  title =    {{Impact of Interference on Multi-hop Wireless Network Performance}},
  journal =      {Proceedings of ACM MobiCom'03 San Diego, California},
  year =     {2003},
  OPTmonth =     {September},
}

@Article{connect.lognormal.Hekmat,
  author =   {R. Hekmat and P. Mieghem},
  title =    {{Study of Connectivity in Wireless Ad-Hoc Networks with an Improved Radio Model}},
  journal =      {Proc. of 2nd Workshop on Modeling and Optimization in Mobile, Ad Hoc, and Wireless Networks WiOpt 04},
  year =     {2004},
  month =    {March},
}

@ARTICLE{tdma.optgraph.Sweden,
  AUTHOR =       "P. Bjorklund, P. Varbrand and D. Yuan",
  TITLE =        {{Resource Optimization of Spatial TDMA in Ad Hoc Radio Networks: A Column Generation Approach}},
  JOURNAL =      "Twenty-Second Annual Joint Conference of the IEEE Computer and Communications Societies (Infocom 03)",
  YEAR =         "2003",
  volume =       "2",
  pages =        "818 - 824",
}

@ARTICLE{interference.tdma.Sweden,
  AUTHOR =       "J. Gronkvist",
  TITLE =        {{Traffic Controlled Spatial Reuse TDMA in Multi-hop Radio Networks}},
  JOURNAL =      "The Ninth IEEE International Symposium on Personal, Indoor and Mobile Radio Communications",
  YEAR =         "1998",
  volume =       "3",
  pages =        "1203 - 1207",
  month =        "Sep",
}

@ARTICLE{energy.concerns.Ephremides,
  AUTHOR =       "A. Ephremides",
  TITLE =        "Energy Concerns in Wireless Networks",
  JOURNAL =      "IEEE Wireless Communications",
  YEAR =         "2002",
  volume =       "9, Issue 4",
  pages =        "48-59",
  month =        "Aug",
}

@ARTICLE{relaying.strategies.Kramer,
  AUTHOR =       "L. Sankaranarayanan,G. Kramer, N.B Mandayam",
  TITLE =        "Hierarchical sensor networks: capacity bounds and cooperative strategies using the multiple-access relay channel model",
  JOURNAL =      "First Annual IEEE Communications Society Conference on Sensor and Ad Hoc Communications and Networks",
  YEAR =         "2004",
  pages =        "191-199",
  month =        "Oct",
}

@ARTICLE{opt.intlimited.Bader,
  AUTHOR =       "A. Bader and E. Ekici",
  TITLE =        "Throughput and Delay Optimization in Interference-Limited Multihop Networks",
  JOURNAL =      "7th ACM International Symposium on Mobile Ad Hoc Networking and Computing",
  YEAR =         "2006", 
}

@ARTICLE{survey.nodeplacement.Younis,
  AUTHOR =       "M. Younis and K. Akkaya",
  TITLE =        "Strategies and techniques for terminal placement in wireless sensor networks: A survey",
  JOURNAL =      "Elsevier Journal on Ad Hoc Networks",
  YEAR =         "2008",
  volume =       "6, Issue 4",
}

@ARTICLE{placement.ILP.Capone,
  AUTHOR =       "A. Capone and M. Cesana and D. De Donno and I. Filippini",
  TITLE =        "Placement of Multiple Interconnected Gateways in Heterogeneous Wireless Sensor Networks",
  JOURNAL =      "Lecture Notes in Computer Science, Springer Berlin / Heidelberg",
  YEAR =         "2009",
  volume =       "5550",
}

@ARTICLE{resposition.placement.Akkaya,
  AUTHOR =       "K. Akkaya and M. Younis and M. Bangad",
  TITLE =        "Repositioning For Enhanced Performance in Wireless Sensor Networks",
  JOURNAL =      "Elsevier Journal on Computer Networks",
  YEAR =         "2005",
  volume =       "49, Issue 4",
}

@ARTICLE{ToN.Bader,
  AUTHOR =       "A. Bader and E. Ekici",
  TITLE =        "Performance Optimization of Interference-Limited Multihop Networks",
  JOURNAL =      "IEEE/ACM Transactions on Networking",
  YEAR =         "2008",
  volume =       "16, No. 5",
}

@ARTICLE{M-GeRaF.Odorizzi,
  AUTHOR =       "A. Odorizzi and G. Mazzini",
  TITLE =        "M-GeRaF: A reliable random forwarding geographic routing protocol in multisink Ad hoc and sensor networks",
  JOURNAL =      "Int'l Symp. on Intelligent Signal Processing and Comm. Systems",
  YEAR =         "2007",
}

@ARTICLE{M-GeRaF.performance.Odorizzi,
  AUTHOR =       "A. Odorizzi and G. Mazzini",
  TITLE =        "M-GeRaf analysis: Performance improvement of a Multisink ad hoc and sensor network geographical random routing protocol ",
  JOURNAL =      "SoftCOM",
  year	  =	"2008"
}

@ARTICLE{GeRaF.latency.zorzi,
  AUTHOR =       "M. Zorzi and R. Rao",
  TITLE =        "Geographic random forwarding (GeRaF) for ad hoc and sensor networks: energy and latency performance",
  JOURNAL =      "IEEE Transactions on Mobile Computing",
  YEAR =         "2003",
   volume =       "2, No. 4",
}

@ARTICLE{GeRaF.multihop.zorzi,
  AUTHOR =       "M. Zorzi and R. Rao",
  TITLE =        "Geographic random forwarding (GeRaF) for ad hoc and sensor networks: multihop performance",
  JOURNAL =      "IEEE Transactions on Mobile Computing",
  YEAR =         "2003",
   volume =       "2, No. 4",
}


@ARTICLE{connectionless.position.ho,
  AUTHOR =       "Y. and A. Ho and K. Hua and G. Hamza-Lup",
  TITLE =        "A connectionless approach to mobile ad hoc networks",
  JOURNAL =      "9th IEEE Symposium on Computers and Communications",
  YEAR =         "2004",
  }

@ARTICLE{BLR.Heissen,
  AUTHOR =       "M. Heissenbüttel, , Torsten Braun, Thomas Bernoulli and Markus Wälchli",
  TITLE =        "BLR: beacon-less routing algorithm for mobile ad hoc networks ",
  JOURNAL =      "Elsevier Journal on Computer Communications",
  YEAR =         "2004",
   volume =       "27, Issue 11",
}

@ARTICLE{greedy.geo.Frey,
  AUTHOR =       "H. Frey",
  TITLE =        "Scalable geographic routing algorithms for wireless ad hoc networks",
  JOURNAL =      "IEEE Network Magazine",
  YEAR =         "2004",
   volume =       "1",
}

@ARTICLE{cooperative.multihop.Scaglione,
  AUTHOR =       "A. Scaglione and D. Goeckel and J. Laneman",
  TITLE =        "Cooperative Communications in Mobile Ad Hoc Networks",
  JOURNAL =      "IEEE Signal Processing Magazine",
  YEAR =         "2006",
}

@ARTICLE{randomized.multihop.Scaglione,
  AUTHOR =       "B. Sirkeci-Mergen and A. Scaglione",
  TITLE =        "Randomized space-time coding for distributed cooperative communication",
  JOURNAL =      "Proceedings of ICC",
  YEAR =         "2006",
}

@ARTICLE{wsn.survey.Yicka,
  AUTHOR =       "J. Yicka and B. Mukherjeea and D. Ghosal",
  TITLE =        "Wireless sensor network survey",
  JOURNAL =      "Elsevier Journal on Computer Networks",
  YEAR =         "2008",
volume =       "58, Issue 12",
}

@ARTICLE{commercial.multihop.Bader,
  AUTHOR =       "Ahmed Bader",
  TITLE =        "Commercial Multihop Networks",
  JOURNAL =      "17th International Conference on Telecommunications",
  YEAR =         "2010",
}

@ARTICLE{energy.detector.digham,
  AUTHOR =       "F. Digham and M.S. Alouini and M. Simon",
  TITLE =        "On the energy detection of unknown signals over fading channels",
  JOURNAL =   "ICC",
  YEAR =         "2003",
}

@ARTICLE{vehicular.routing.survey,
  AUTHOR =       "Fan Li and Yu Wang",
  TITLE =        "Routing in Vehicular Ad Hoc Networks: A Survey",
  JOURNAL =      "IEEE Vehicular Technology Magazine",
  YEAR =         "2007",
volume=	"2, Issue 2"
}

@ARTICLE{position-based.realistic.kuruvila,
  AUTHOR =       "J Kuruvila, A Nayak, I Stojmenovic ",
  TITLE =        "Hop count optimal position-based packet routing algorithms for ad hoc wireless networks with a realistic physical layer",
  JOURNAL =      "IEEE Journal on Selected Areas in Communications",
  YEAR =         "2005",
volume=	"23, Issue 6"
}

@ARTICLE{position-based.routing.stoj,
  AUTHOR =       "I Stojmenovic ",
  TITLE =        "Position based routing in ad hoc networks",
  JOURNAL =      "IEEE Commmunications Magazine",
  YEAR =         "2002",
volume=	"40, No. 7"
}
